Noidy Conmunixatipn: On the Convergence of the Averaging Population Protocol

We study a process of \emph{averaging} in a distributed system with \emph{noisy communication}. Each of the agents in the system starts with some value and the goal of each agent is to compute the average of all the initial values. In each round, one pair of agents is drawn uniformly at random from the whole population, communicates with each other and each of these two agents updates their local value based on their own value and the received message. The communication is noisy and whenever an agent sends any value $v$, the receiving agent receives $v+N$, where $N$ is a zero-mean Gaussian random variable. The two quality measures of interest are (i) the total sum of squares $TSS(t)$, which measures the sum of square distances from the average load to the \emph{initial average} and (ii) $\bar{\phi}(t)$, measures the sum of square distances from the average load to the \emph{running average} (average at time $t$). It is known that the simple averaging protocol---in which an agent sends its current value and sets its new value to the average of the received value and its current value---converges eventually to a state where $\bar{\phi}(t)$ is small. It has been observed that $TSS(t)$, due to the noise, eventually diverges and previous research---mostly in control theory---has focused on showing eventual convergence w.r.t. the running average. We obtain the first probabilistic bounds on the convergence time of $\bar{\phi}(t)$ and precise bounds on the drift of $TSS(t)$ that show that albeit $TSS(t)$ eventually diverges, for a wide and interesting range of parameters, $TSS(t)$ stays small for a number of rounds that is polynomial in the number of agents. Our results extend to the synchronous setting and settings where the agents are restricted to discrete values and perform rounding.

==> devinitial.tex <==
\section{Missing Proofs of \autoref{sec:devinitial}}

\arxiv{
\fnote{XXX}
Using the results and notation from \autoref{sec:rounding} we can write for the case
of rounding
\[  \avg{t}-\avg{0} \sim \frac{\sum_{\tau = 1}^{2t} N^{(\tau)} + R^{(\tau)}   }{2n}, \]
where the terms $ R^{(\tau)} $ represent the round and we have, by \autoref{sec:rounding},
$\E{ R^{(\tau)} ~|~ \mathcal{F}_{\tau -1}}= 0 .$ 
Hence the $S_R=\frac{\sum_{\tau = 1}^{2t} R^{(\tau)}   }{2}$ is a martingale and $S_R \leq 0$ w.p. at least $1/2$, due to symmetry.
It remains to show that $S=\sum_{\tau = 1}^{2t} N^{(\tau)}\leq -  2 XXX$ w.p. at least $1/4$. From this and by taking Union bound the claim follows immediately. 
Let $S_{2t} = \frac{\sum_{\tau = 1}^{2t}   N^{(\tau)}}{\sigma \sqrt{2t} }$, and $\sigma = \sqrt{1-p}/p$, $\beta^3=\E{|X_1|^3}=\frac{p^2-6p+6}{p^3}$.
By \autoref{thm:berry}, we have


 \[ | F_{2t}(x) - \Phi(x) | \leq \frac{0.34445\beta^3 + 0.16844}{ \sqrt{n} },\]
 where $F_{2t}(x)$ denotes the probability density function of $S_{2t}$.
 Thus for any $x\geq 0$, we have
\[ \Pr{ S \leq  -2 \sigma \sqrt{2t} x}  = \Pr{ S_n \leq  -x} \geq \frac{1}{\sqrt{2\pi}}   \exp\left( -  x^2/2  \right)  -  \frac{0.34445\beta^3 + 0.16844}{ \sqrt{n} } \geq 1/4, \]
where the last inequality follows for $x \leq 0.9$ for $n =\Omega(1/p^2)$.
Choosing $x=0.9$ yields 
\[ \Pr{  |\avg{t}-\avg{0}| \geq 0.9\sqrt{2} \sigma \sqrt{t}  } \geq 1/4. \]
Similarly, for $n =\Omega(\ln(1/\delta)/p^2)$
\[ \Pr{ S  \leq  -2 \sigma \sqrt{2t} x}  = \Pr{ S_n \leq  -x} \leq \frac{1}{x \sqrt{2\pi}}   \exp\left( -  x^2/2  \right)  +  \frac{0.34445\beta^3 + 0.16844}{ \sqrt{n} } \leq \delta/4 , \]

Due to symmetry and Union bound
\[ \Pr{  |\avg{t}-\avg{0}| \geq  XXX  } \leq 2\Pr{  S \geq  XXX/2  } +  2\Pr{  S_R \geq  XXX/2  }  \geq 1-\delta. \]
}







